Introducing MANtIS: a novel Multi-Domain Information Seeking Dialogues Dataset

Conversational search is an approach to information retrieval (IR), where users engage in a dialogue with an agent in order to satisfy their information needs. Previous conceptual work described properties and actions a good agent should exhibit. Unlike them, we present a novel conceptual model defined in terms of conversational goals, which enables us to reason about current research practices in conversational search. Based on the literature, we elicit how existing tasks and test collections from the fields of IR, natural language processing (NLP) and dialogue systems (DS) fit into this model. We describe a set of characteristics that an ideal conversational search dataset should have. Lastly, we introduce MANtIS (the code and dataset are available at https://guzpenha.github.io/MANtIS/), a large-scale dataset containing multi-domain and grounded information seeking dialogues that fulfill all of our dataset desiderata. We provide baseline results for the conversation response ranking and user intent prediction tasks.

==> sections/table-mantis.tex <==
\setlength{\extrarowheight}{3pt}
\begin{table*}[htb]
    \centering
    \tiny
    \begin{tabular}{@{}L{1.2cm}L{11cm}L{2.5cm}@{}}
    \toprule
    \textbf{Domain}  &  \textbf{Example conversation} & \textbf{Utterance labels}\\
    \midrule
    \multirow{5}{*}{apple}
    & \colorbox{lightgray}{- I want a firewall that will protect me but more of that to monitor any connection in or out of my mac...} 
    & Original Question \\ \cline {2-3}
    & - That would be the \colorbox{yellow}{TCPblock \{url removed\}} ... With TCPBlock you can prevent selected applications on your computer from opening connections to the network & Potential Answer \\ \cline{2-3}
    & - Thank you. This app is not from identified developer it is safe to use it? ...
    & Greeting / Gratitude \newline Information Request \\ \cline{2-3}
    & - I understand, but there is nothing that it 100\% safe and I use it ...
    & Further Details \\ \cline{2-3}
    & - Cheers anyway! I will try to buy ... which is more safe ...
    & Greeting / Gratitude \\
    \midrule
    \multirow{7}{*}{askubuntu}
    & - I'm unable to install any of the programs from Ubuntu Software Center. It constantly stays at 0\% with the following message ...
    & Original Question \\ \cline{2-3}
    & - \colorbox{pink}{Do you have synaptic or the ubuntu software center open?} .. If no synaptic processes are running, type the following in terminal.. Also see \colorbox{yellow}{ this \{url removed\}}... 
    & Information Request \newline Potential Answer \\ \cline{2-3}
    & - Thank you for help! There were no synaptic processes. Where exactly do i need to type?
    & Greetings / Gratitude \newline Information Request \\ \cline{2-3}
    & - In terminal. To open terminal go to... 
    & Further Details \\ \cline{2-3}
    & - Ok, I did. Now I have this message..
    & Further Details \\ \cline{2-3}
    & - Type `sudo apt-get update`
    & Further Details \\ \cline{2-3}
    & - \colorbox{green}{Wonderful! It worked} ...
    & Positive Feedback \\
    \midrule
    \multirow{4}{*}{electronics}
    & - \colorbox{lightgray}{Can a PIC32MZ have multiple SPI ports running at the same time? If so, how?} ...
    & Original Question \\ \cline{2-3}
    & - Yes. According to the \colorbox{yellow}{PIC32MZ Embedded Connectivity Family  datasheet \{url removed\}, page 1}, it has "Six 4-wire SPI modules" ....
    & Potential Answer \\ \cline{2-3}
    & - Okay, I understand that now.  Now I need to understand the program flow ...
    & Positive Feedback \newline Follow Up Question \\ \cline{2-3}
    & - Yes, if you want help with program flow, ask a new question ....
    & Potential Answer \\
    \bottomrule
    \end{tabular}
    \caption{\dataset{} conversation examples. {\small\colorbox{yellow}{Yellow}} shows document grounding, {\small\colorbox{green}{green}} displays final positive message from the original poster, {\small\colorbox{pink}{pink}} are clarification questions and {\small\colorbox{lightgray}{gray}} highlights initial information needs. All examples in the table are multi-turn. The right-most column shows the conversation labels for each utterance.}
    \label{tab:sites}
\end{table*}
